Efficient Butterfly Counting for Large Bipartite Networks

Bipartite networks are of great importance in many real-world applications. In bipartite networks, butterfly (i.e., a complete 2 x 2 biclique) is the smallest non-trivial cohesive structure and plays a key role. In this paper, we study the problem of efficient counting the number of butterflies in bipartite networks. The most advanced techniques are based on enumerating wedges which is the dominant cost of counting butterflies. Nevertheless, the existing algorithms cannot efficiently handle large-scale bipartite networks. This becomes a bottleneck in large-scale applications. In this paper, instead of the existing layer-priority-based techniques, we propose a vertex-priority-based paradigm BFC-VP to enumerate much fewer wedges; this leads to a significant improvement of the time complexity of the state-of-the-art algorithms. In addition, we present cache-aware strategies to further improve time efficiency while theoretically retaining the time complexity of BFC-VP. Moreover, we also show that our proposed techniques can work efficiently in external and parallel contexts. Our extensive empirical studies demonstrate that the proposed techniques can speed up the state-of-the-art techniques by up to two orders of magnitude for the real datasets.

==> 5related_works.tex <==
\vspace{-0.3cm}
\section{Related Work}
\vspace{-0.1cm}
\label{sct:related}
\noindent
{\bf Network motif counting.}
%Network motif counting has been widely studied in many applications such as network measurement \cite{hu2013massive}, graph decomposition \cite{sariyuce2018peeling}, and research of replacement \cite{palmer1983broken, ornstein1984interlocking, ornstein1982interlocking}.
In unipartite networks, as triangle is the smallest non-trivial cohesive structure, there exist extensive studies on counting triangles in literature  \cite{chang2017scalable, becchetti2008efficient, schank2005finding, kolountzakis2012efficient, chu2012triangle, seshadhri2013triadic, stefani2017triest, shun2015multicore, al2018triangle, hu2013massive, latapy2008main, itai1978finding, alon1997finding, schank2005finding, suri2011counting}.  However,  these works cannot be applied to solve our butterfly counting problem. This is because the state-of-the-art triangle counting algorithms need $O(m^{1.5})$ time to enumerate all the triangles and the number of butterflies in bipartite networks can scale to $\Theta(m^2)$ which cannot afford to do the enumerating. In addition, some studies \cite{jain2017fast, pinar2017escape, jha2015path} focused on the other cohesive structures such as 4-vertices and 5-vertices, their algorithms also cannot be used to solve our problem.
%In addition, the number of triangles in unipartite networks is bounded by $O(m^{1.5})$ while the number of butterflies in bipartite networks can scale to $\Theta(m^2)$ which is more challenging to count.

In bipartite networks, some works tried to define motifs as $3 \times 3$ biclique \cite{borgatti1997network} and 4-path \cite{opsahl2013triadic}. These structures are different with the butterfly thus these works also cannot be used to solve the butterfly counting problem. Recent works in \cite{wang2014rectangle, sanei2018butterfly} studied the butterfly counting problem in bipartite networks.  Wang et al. in \cite{wang2014rectangle} studied exact butterfly counting algorithms including in-memory, distributed, and I/O efficient versions.
In \cite{sanei2018butterfly}, the authors proposed an improved exact algorithm to compute $\btf_G$ and the randomizing-based approximate algorithms to estimate $\btf_G$. Our proposed \newa algorithm significantly outperforms the exact butterfly counting algorithms proposed in \cite{wang2014rectangle, sanei2018butterfly}. Furthermore, we can speed up \bsap using \newa because \bsap deploys exact butterfly counting as an essential procedure.

%Although these metrics are useful in some fields, the butterfly is still the smallest non-trivial biclique in bipartite networks and plays the same key role as the triangle in uniparite networks. In addition, t Our proposed \newa algorithm achieves a similar performance with their most efficient edge-specification-based algorithm \bsap.


%But the time complexity of their algorithm is still $O(m^2)$.
% the most recent related work
%the total number of butterflies (i.e., $\btf_G$) in $G$
%These algorithms cannot count or even estimate the number of butterflies containing each edge (i.e., $\btf_e$) in $G$.
%Their proposed algorithm outperforms the matrix-multiplication-based methods for counting cycles in a graph \cite{alon1997finding}.
%% including in-memory, parallel, I/O efficient versions By processing the wedges from each vertex in one of a vertex layer, their algorithm can count the number of butterflies in $O(m^2)$ time complexity.


\noindent
{\bf Graph ordering.} In literature, many recent works studied graph ordering to speed up graph algorithms. Some works \cite{wei2016speedup, blandford2003compact, chierichetti2009compressing, dhulipala2016compressing, tatikonda2009efficient, kang2011beyond, auroux2015reordering, boldi2009permuting, boldi2011layered} focused on general graph ordering methods. In \cite{blandford2003compact, chierichetti2009compressing, dhulipala2016compressing, tatikonda2009efficient, kang2011beyond, boldi2009permuting, boldi2011layered}, the authors studied graph compression to reduce the number of bits of edges. Wei et al. \cite{wei2016speedup} recently proposed a general method to reduce the cache miss ratio in graph algorithms. In our experiments, we compare our graph projection strategy with the state-of-the-art general method in \cite{wei2016speedup}. Some works focused on improving specific graph algorithms using graph ordering. Then et al. optimized BFS algorithm in \cite{then2014more}. Park et al. in \cite{park2004optimizing} improved the CPU cache performance of many classic graph algorithms such as Bellman-Fold and Prim. The authors in \cite{han2018speeding} presented a suite of approaches to accelerate set intersections in graph algorithms.
%Their work cannot be applied here because the set intersection operations are not needed in the proposed butterfly counting algorithms. graph ordering

